AdaSlicing: Adaptive Online Network Slicing under Continual Network Dynamics in Open Radio Access Networks

Open radio access networks (e.g., O-RAN) facilitate fine-grained control (e.g., near-RT RIC) in next-generation networks, necessitating advanced AI/ML techniques in handling online resource orchestration in real-time. However, existing approaches can hardly adapt to time-evolving network dynamics in network slicing, leading to significant online performance degradation. In this paper, we propose AdaSlicing, a new adaptive network slicing system, to online learn to orchestrate virtual resources while efficiently adapting to continual network dynamics. The AdaSlicing system includes a new soft-isolated RAN virtualization framework and a novel AdaOrch algorithm. We design the AdaOrch algorithm by integrating AI/ML techniques (i.e., Bayesian learning agents) and optimization methods (i.e., the ADMM coordinator). We design the soft-isolated RAN virtualization to improve the virtual resource utilization of slices while assuring the isolation among virtual resources at runtime. We implement AdaSlicing on an O-RAN compliant network testbed by using OpenAirInterface RAN, Open5GS Core, and FlexRIC near-RT RIC, with Ettus USRP B210 SDR. With extensive network experiments, we demonstrate that AdaSlicing substantially outperforms state-of-the-art works with 64.2% cost reduction and 45.5% normalized performance improvement, which verifies its high adaptability, scalability, and assurance.

==> motivation.tex <==
\section{Background and Motivation.}

\textbf{Background.}
Network slicing
RAN virtualization


\textbf{Motivation.}
slice comes and goes -- > adaptability
slice needs non-stationary by time-varying --> online learning 
resource utilization low in hard isolation --> soft isolation


Under the growing trend of network slicing, Mobile Network Operators(MNO) aim to orchestrate resources to minimize operational costs while meeting the performance requirements of users within each slice. In traditional networks, MNO customize a dedicated network for users based on specific needs, such as low latency and high throughput. However, once user demands change, such as service upgrades requiring higher throughput, operators need to expand the physical network infrastructure to accommodate these changes. Furthermore, the increasing complexity of applications demands more precise and sophisticated network performance, necessitating a shift in resource orchestration from a one-size-fits-all approach to a one-size-per-service model. This forces MNO to invest more in the establishment of network infrastructure and the design of dedicated networks.

Network slicing allows a physical network infrastructure to be divided into multiple logically independent virtual networks. Each network slice is an isolated end-to-end network with its unique characteristics in terms of latency, throughput, and bandwidth, which can flexibly cater to diverse requirements and services. As a result, network slicing technology can significantly reduce costs. However, existing slicing techniques still do not effectively improve the utilization of wireless resources. Typically, for a given slice, its network resources are generally fixed and cannot be dynamically adjusted based on the actual traffic and resource usage within the application. For example, an application within a slice may have no traffic at certain times, while at the same time, another slice might request network resources exceeding the maximum capacity. Such scenarios lead to wasted radio resources in the network, resulting in unnecessary expenses for mobile operators, and can adversely affect the quality of service for applications. In this context, we propose an adaptive dynamic network slicing technique that dynamically orchestrates the radio resources across slices online, minimizing the cost of mobile operators while satisfying the network requirements of applications.

Overall, there are three main challenges in applying adaptive dynamic network slicing techniques to real-work networks. The first challenge is the discrepancy between the resources demanded by slices and those allocated to slices. This leads to hard isolation slicing techniques being unable to flexibly respond to changing resource requests. The second challenge concerns how to allocate surplus resources within certain slices based on the priority of applications, while still ensuring network performance meets the requirements of all applications. Additionally, when adaptively orchestrating wireless resources within network slices, the status of other slices and whether the allocation could potentially conflict with the performance of these other slices should be considered.

% motivation
\textbf{Demand-to-allocated resources discrepancy.} Different applications impose a variety of Quality of Service (QoS) requirements on the network. Hard isolation policies provide each slice instance with exclusive, non-shared resources, apparently ensuring the required performance, availability, and reliability for each application or customer. However, the reality is that dedicated and static isolation can lead to wastage of network resources. For instance, if resources within a slice remain underutilized, they cannot be allocated to other slices. Moreover, static allocation fails to accommodate sudden surges in traffic, resulting in the inability to fulfill services that exceed the assigned slice capabilities. This discrepancy between the demand for and allocation of network resources necessitates the development of a dynamic isolation approach that allows for the adjustment and sharing of network resources.

\textbf{Different task priorities.} In network communications, tasks have varying priorities.Time-sensitive applications, such as vehicular networks and industrial control, require millisecond-level latency, posing challenges to network bandwidth. Similarly, tasks like live streaming and video transmission demand high bandwidth. Obviously, these tasks differ in importance. Additionally, users may be willing to pay to prioritize their tasks, thereby utilizing more network resources. Slices with spare resources could sell their capacity, enhancing resource utilization for operators. From the perspective of network resource allocation, we propose a weighted distribution of shared resources.

\textbf{Constraint violation.} Challenges arise when slices adjust their weights to request allocation of shared resources. This adjustment can potentially affect the performance of applications within the slice. The allocation strategy should primarily fulfill the needs of users within a slice under hard isolation conditions, addressing factors such as latency and throughput. Only after ensuring that these performance criteria are not compromised, the remaining network resources could be redirected to a shared resource pool for use by slices experiencing resource shortages. Consequently, an online approach is necessary to interact and learn weight request strategies from the real network environment, which consider the status of all slices.
%\textbf{Demand-to-allocated resources discrepancy.}
%why soft isolation(disadvantage of the hard isolation)
%\textbf{Different task priorities.}
%why weighted allocation
%\textbf{Constraint violation.}
%System state
%why allocation algorithm, we consider the state of other slicing

